Octopus: Privacy-Preserving Collaborative Evaluation of Loan Stacking

With the rise of online lenders, the loan stacking problem has become a significant issue in the financial industry. One of the key steps in the fight against it is the querying of the loan history of a borrower from peer lenders. This is especially important in markets without a trusted credit bureau. To protect participants privacy and business interests, we want to hide borrower identities and lenders data from the loan originator, while simultaneously verifying that the borrower authorizes the query. In this paper, we propose Octopus, a distributed system to execute the query while meeting all the above security requirements. Theoretically, Octopus is sound. Practically, it integrates multiple optimizations to reduce communication and computation overhead. Evaluation shows that Octopus can run on 800 geographically distributed servers and can perform a query within about 0.5 seconds on average.

==> secure_comparison.tex <==
\section{Secure Evaluation}
\label{section:secure_comparison}

The next key stage is to enable the borrower and the originator collaboratively evaluate the query of the form in Eq.~\ref{equation:query} while preserving everyone's privacy.
% In this paper, this means that the borrower should prove to the originator that $\sum x_i < t$ without revealing $x = \sum x_i$ and $x_i$'s to the originator, while the originator keeps the threshold $t$ private.
As the borrower has sent a commitment to $x$ to the originator for consistency check (see Protocol~\ref{protocol:pir_sparse_recursive}), the concrete goal of this section is to provide an approach that outputs the evaluation result of Eq.~\ref{equation:query} using the commitment $c$, the originator's private data $t$ and the public paramter $\theta$.
In \sysname, we use ZKP and non-interactive actively secure computation (NISC)~\cite{NISC} to achieve this goal. 
Note that, although all the communication between the borrower and the originator is through the exchanger, we ommit the exchanger in this section for simplicity, as the exchanger only performs message relayer in the following discussions.
In this paper, we present how \sysname supports the following queries:

\para{Sum.}
The sum query helps the originator get the sum of $\tilde{x}_i$.
The support for sum query is direct, as the originator has collected commitments which support homomorphic addition. 
Thus, \sysname only needs to set $f'$ in Eq.~\ref{equation:query} as the trivial function $f'(x) = x$, and then the borrower opens the aggregated commitment $c$ in Protocol~\ref{protocol:pir_sparse_recursive} to reveal $\sum \tilde{x}_i$ to the originator.

\para{Count.}
The count query tells the originator how many lenders has lent money to the borrower. \sysname sets $f'$ as the boolean function: $f'(x) = 1$ if $x > 0$ otherwise $f'(x) = 0$.
The remaining process for aggregating the boolean values is similar as the sum query.

\para{Variance.}
The variance of $\tilde{x}_i$'s can be calculated as $(\frac{1}{n}\sum_i\tilde{x}_i^2) - (\frac{1}{n}\sum_i\tilde{x}_i)^2$.
Intuitively, the originator can first collect the commitment to $\sum_i\tilde{x}_i^2$ (which we denote as $F_1$) and the commitment to $(\sum_i\tilde{x}_i)^2$ (which we denote as $F_2$), then the originator calculates $F_3 = F_1^n F_2^{-1}$, which is the commitment to $(n\sum_i\tilde{x}_i^2) - (\sum_i\tilde{x}_i)^2$, and opens $F_3$ with the help of the borrower.
The originator can easily obtain $F_1$ by setting $f'(x) = x^2$. However, it is not direct to get $F_2$ using the commitments from the lenders, as the commitment scheme is not multiplicatively homomophic. To solve this, we use the \emph{multiplication ZKP} in \cite{ZKP_HOMO}, which proves that a number hidden in a commitment is the product of the two numbers hidden in another two commitments.

Specifically, to get the commitment to $(\sum_i\tilde{x}_i)^2$, the originator first uses Protocol~\ref{protocol:pir_sparse_recursive} to retrieve the commitment to $\sum_i \tilde{x}_i$ (which we denote as $F_4$), while the borrower sends $F_2$ (i.e. the commitment to $(\sum_i\tilde{x}_i)^2$) along with the proof which proves that the number hidden in $F_2$ is the square of the number hidden in $F_4$ to the originator. Once the originator verifies that $F_2$ is the commitment to $(\sum_i\tilde{x}_i)^2$, it can obtain the variance using $F_1$ and $F_2$, as shown above.

\para{Comparison with a public number.}
Sometimes an auditor wants to check whether a borrower has borrowed money from too many lenders to evaluate the credit of that borrower.
For example, if a borrower has borrowed money from more than 5 lenders, the borrower may be forbidden to borrow money anymore until she has paid off her loans.
Note that this kind of query is different from the count query, as the count query reveals the exact number of lenders that have lent money to the borrower, while this kind of query only reveals a boolean value which indicates the count is greater than a public number or not without revealing the exact count.
To achieve this goal, we use the \emph{interval ZKP}~\cite{INTERVAL_ZKP}, which proves that a committed number lies in a public interval.
The interval ZKP is efficient and non-interactive. In \sysname, the borrower sends the proof to the originator and then the originator verifies the proof to get the comparison result.

\para{Comparison with a private number.}
It is common that a loan company will not lend money to a borrower who has borrowed too much money from others. 
On the other hand, the loan company may set different thresholds for different borrowers and is not willing to reveal the thresholds to anyone else, as the borrower ratings are commercial secrets 
In this case, the loan company acts as the originator and issues a query to collect the loan information of the borrower.
Specifically, the originator set $f$ in Eq.~\ref{equation:query} as the comparison result of $\sum_i \tilde{x}_i < t$, where $t$ is a private threshold only known by the originator.
A direct approach for such secure comparison is \emph{garbled circuit (GC)}~\cite{GC}. The original GC assumes two semi-honest players. However, in our situation, both the borrower and the originator have the motivation to deviate from the protocol to cheat or steal private information. We thus use the \emph{non-interactive actively secure computation (NISC)} scheme in \cite{NISC} to support such query.

The above NISC scheme provides active security for GC using \emph{cut-and-choose}~\cite{CUT_AND_CHOOSE}. Also, we employ common optimizations for GC, such as \emph{free-xor}~\cite{FREE_XOR} and \emph{half-and}~\cite{TWO_HALVES}.
And we have a micro modification: although the protocol in \cite{NISC} generates input commitments to prove the consistency of inputs of different circuits, in our scenario, however, the originator needs to make sure that the input commitments for secure computation are also consistent with the commitment in the consistency check stage (see Protocol~\ref{protocol:pir_sparse_recursive}), otherwise the borrower is still able to use a fake input for secure comparison to cheat the originator. 
Thus in \sysname, the borrower also needs to prove the consistency. 
Specifically, in \cite{NISC}, the circuit generator (namely the borrower in this paper) generates an input commitment $c_j$ for the $j$-th bit of her input.
Then the borrower in \sysname generate proofs for two things:
a) each $c_j$ commits either $0$ or $1$;
b) $c = \prod c_j^{2^j}$ commits the same number as the commitment $c_b$ in Protocol~\ref{protocol:pir_sparse_recursive}. 
The borrower sends the proofs to the originator through the exchanger, and the originator verifies them to get the comparison result.

\begin{comment}
\subsection{Alternative \uromann{1}: Non-Interactive Actively Secure Garbled Circuit}
\label{section:nisc}

The basic idea of this alternative is to use secure multi-party computation (SMC) to perform comparison without revealing each participant's private data to others. 
We use garbled circuit (GC)~\cite{GC} to perform secure comparison. The original protocol in \cite{GC} assumes that the two players are semi-honest and would follow the protocol.
However, in our scenario, to get loan from the originator, the borrower may use fake input or generate invalid ciruit to cheat the originator, while the originator may also try to infer extra information about the borrower's input during the computation. 
Thus, the solution should provide \emph{active security} aganist malicious participants.
Moreover, as mentioned in Section~\ref{section:architecture}, the communication between the originator and the borrower should be non-interactive. 

The paper \cite{NISC} proposes a non-interactive secure computation protocol, which provides active security using \emph{cut-and-choose}~\cite{CUT_AND_CHOOSE}.
We use the protocol in \cite{NISC} for secure comparison, and employ common optimizations for GC, such as \emph{free-xor}~\cite{FREE_XOR} and \emph{half-and}~\cite{TWO_HALVES}. 
Also, we have a micro modification: although the protocol in \cite{NISC} generates input commitments to prove the consistency of inputs of different circuits, in our scenario, however, the originator need to make sure that the input commitments for secure comparison are also consistent with the commitment in the consistency check stage (see Protocol~\ref{protocol:pir_sparse_recursive}), otherwise the borrower is still able to use a fake input for secure comparison to cheat the originator. 
Thus in \sysname, the borrower also needs to prove the consistency. 
Specifically, in \cite{NISC}, the circuit generator (namely the borrower in this paper) generates an input commitment $c_j$ for the $j$-th bit of her input.
Then the borrower in \sysname generate proofs for two things:
a) each $c_j$ commits either $0$ or $1$;
b) $c = \prod c_j^{2^j}$ commits the same number as the commitment $c_b$ in Protocol~\ref{protocol:pir_sparse_recursive}. 
The borrower sends the proofs to the originator through the exchanger, and the originator verifies them.

\subsection{Alternative \uromann{2}: Interval ZKP}
\label{section:interval_zkp}

The above alternative is straitfoward, but it needs to transfer multiple encrypted circuits, which is bandwidth consuming.
A communication-efficient way is to use zero-knowledge proof to prove that a commited number lies in an interval~\cite{BOUNDEDNESS_ZKP, LENGTH_ZKP, INTERVAL_ZKP, CFT, BCDG}.
However, such ZKP techniques usually require the interval to be known by both the prover and the verifier. This is not the case in \sysname, as the originator (namely the verifier) needs to hide its threshold $t$. 
In \sysname, the borrower first picks an integer $t'$ larger than $x$ and sends $t'$ to the originator before generating the interval ZKP. Then, instead of proving $x < t$ directly, the borrower uses the commitment $c = F(x)$ and the intermediate threshold $t'$ to generate the zero-knowledge proof which proves that the number $x$ hidden in $c$ is in the interval $[0, t']$. Thus, as long as $t' < t$ and the above proof is correct, the originator can make sure that $x < t$. 

To prove that a committed number lies in a public interval (i.e. $x \in [0, t']$), we use the interval ZKP technique in \cite{INTERVAL_ZKP}, which is non-interactive and efficient both in terms of computation and communication. 
On the other hand, as the borrower does not know the exact value of $t$, how to choose the value of $t'$ is tricky: a large $t'$ causes failure when $t' > t$, while a small $t'$ reveals too much information about $x$ to the originator, as a small upper bound of $x$ narrows the possible range of $x$. 
Therefore, while choosing a proper value for $t'$, there is a trade-off between privacy and risk of a wrong result.

Compared with the alternative based on NISC, this protocol requires the borrower to know the interval during the computation, and the borrower needs to send a $t'$ to the originator, which may reveal extra information about the borrower's input. On the other hand, NISC uses garbled circuit and employs cut-and-choose to achieve active security, thus causes higher communication and computation cost.
In practice, we should make a right trade-off when we make a choice between these two alternatives.

\end{comment}


==> security_analysis_ideal_sim.tex <==
\section{Security Analysis and Proof of \sysname}
\label{appendix:formal_proof}
In this appendix, we prove the overall security of \sysname, by proving that each role does not see any private information that is not supposed to be revealed to it. Then we argue that these security properties satisfy the security requirements in Section~\ref{section:security_goal}.

\subsection{Security Definition}
We first define the functionality $\mathcal{F}_{loan}$ as follows:

\noindent \begin{minipage}[h]{0.47\textwidth}
\fbox{
\parbox{\textwidth}{
\begin{center}
Functionality $\mathcal{F}_{loan}$
\end{center}
    Upon receiving the plaintext of a $d$-dimensional query $q$, the query function $f$, the private input $t$ and the key pair $(sk, pk)$ from the originator, a random number $r_e$, the secrets $s_{eu}$'s shared between the exchanger and the users/borrowers and the random tape $R$ from the exchanger, the secret $s_{eb}$ and the sum $X_b$ from the current borrower, the databases $D_i$'s from the lenders, and the common input $gid_b$ and $N_g$, $\mathcal{F}_{loan}$ does the following:
\begin{enumerate}[leftmargin=0.5cm, label=\arabic*.]
\item Check that the plaintext query $q$ contains only one $1$ in each dimension. If the check succeeds, output $z_1 = ``pass"$ to the exchanger, otherwise output $z_1 = \bot$ to the exchanger and abort.
\item Retrieve the secret from the secrets from the exchanger according to $gid_b$ and the plaintext query $q$, then check that the retrieved secret is consistent with the secret from the borrower. If the check succeeds, output $z_2 = ``pass"$ to the exchanger, otherwise output $z_2 = \bot$ to the exchanger and abort.
\item Retrieve the values $x_{ib}$'s from the databases of lenders using $q$, and encrypt them recursively using the public key of the originator. For each $x_{ib}$, if it equals $0$, sample a random number $i \in \{1, 2, \dots, d\}$ and generate a randomized ciphertext of \type{i}. Otherwise, encrypt it as a ciphertext of \type{0}.
\item Generate noise responses according to Theorem~\ref{thm:differential_privacy} which makes the types of ciphertexts $(\epsilon, \delta)$-differentially private. The randomness is sampled from the random tape $R$ of the exchanger. Then mix and shuffle the noise with the ciphertexts (we denote the set of ciphertexts as $C$). Decrypt these ciphertexts using the originator's private key $sk$ and send the vector $\textbf{n} = (n_0, n_1, \dots, n_d)$ to the originator, where $n_i$ is the number of ciphertexts of \type{i} in $C$.
\item Check that $\sum_i x_{ib}$ equals $X_b$. If the check succeeds, output $z_3 = ``pass"$ to the originator, otherwise output $z_3 = \bot$ to the originator and abort.
\item Calculate the query result $z_4 = f(X_b, t)$ and send $z_4$ to the originator.
\end{enumerate}
}
}
\end{minipage}

$\mathcal{F}_{loan}$ only outputs information necessary to each participant, and hides the information not supposed to be revealed.
Now we define the security of \sysname as follows:

\begin{defi} \label{def:security}
    A protocol $\pi$ securely realizes $\mathcal{F}_{loan}$ in the presence of a semi-honest exchanger that uses the random tape $R$, semi-honest lenders, a malicious borrower and a malicious originator, 
    if for every probabilistic polynomial-time adversary $i \in \{ex, og, bo, le\}$ (which stands for exchanger, originator, borrower and lender, respectively), there exists a probabilistic polynomial-time algorithm $\mathcal{S}_i$ such that for every input tuple $\mathcal{I} = (q, f, t, r_e, s_{eu}\text{'s}, s_{eb}, X_b, D_i\text{'s})$, we have:
\begin{center}
    $\mathcal{S}_{ex}(r_e, s_{eu}\text{'s}, z_1, z_2) \approx \text{View}_{ex}^{\pi}(\mathcal{I})$, \\ % and $\text{Output}_{ex}^{\pi}(\mathcal{I}) = (z_1, z_2)$, \\
    $\mathcal{S}_{og}(q, f, t, \textbf{n}, z_3, z_4) \approx \text{View}_{og}^{\pi}(\mathcal{I})$, \\ % and $\text{Output}_{og}^{\pi}(\mathcal{I}) = (z_3, z_4)$, \\
    $\mathcal{S}_{bo}(s_{eb}, X_b) \approx \text{View}_{bo}^{\pi}(\mathcal{I})$, \\
    $\mathcal{S}_{le}(D_i\text{'s}) \approx \text{View}_{le}^{\pi}(\mathcal{I})$. 
\end{center}
%    where $\approx$ means \emph{computationally indistinguishable}.
\end{defi}

\begin{thm}
\label{thm:correctness}
\sysname securely realizes $\mathcal{F}_{loan}$ in the presence of a semi-honest exchanger, semi-honest lenders, a malicious borrower and a malicious originator. 
\end{thm}

\subsection{Security Analysis}
We have proven the correctness of the outputs in the above sections. In this section, we focus on the security analysis of \sysname.
We show how to construct a simulator for the exchanger and analyze the security of its view. The other participants can be analyzed in a similar way. 

\para{Exchanger. }
The view of the exchanger in the real execution includes three parts:
\begin{enumerate}[label={\alph*)}, leftmargin=0.5cm, itemsep=0pt, partopsep=0pt, parsep=0pt]
    \item During the secure aggregation: an encrypted $d$-dimensional query $q$ from the originator, a ciphertext $c_i$ of \type{j} $(j \in \{0, 2, \dots, d\})$ from each lender $S_i (i = 1, 2, \dots, n)$, a random number $\Delta r$ and a commitment $c_b$ of the sum from the borrower; \\
    \item During the anonymous authorization: a ciphertext $c$ of a pseudo-random number $y$ generated using $r_e$ and the zero-knowledge proof $P_c$ that proves the knowledge of the plaintext of $c$ from the borrower, the zero-knowledge proof $P_{form}$ which proves that the query $q$ is well-formed and the zero-knowledge proof $P_{corr}$ that proves the correspondence of the query and the encrypted secret from the borrower; \\
    \item  During the secure evaluation: the ciphertexts or commitments from the borrower and the originator to evaluate $f$, and we denote them as $\Lambda_{bf}$ and $\Lambda_{of}$, respectively. \\
\end{enumerate}
In summary, the view of the exchanger is the tuple:
$\text{View}_{ex}^{\pi}(\mathcal{I}) = (q, c_i\text{'s}, \Delta r, c_b, c, P_c, P_{form}, P_{corr}, \Lambda_{bf}, \Lambda_{of})$.

We then construct a probabilistic-polynomial time simulator $\mathcal{S}_{ex}$ that simulates the view of the exchanger using its input (namely $r_e$ and $s_{eu}$'s) and output (namely $z_1$ and $z_2$). 
Note that, in this proof, we only consider the situation where the values of $z_1$ and $z_2$ are both $``pass"$. This is because any $\bot$ (i.e. abortion) would actually result in a simpler case and we omit the analysis for such abortion situations.

Specifically, $\mathcal{S}_{ex}$ works as follows:
\begin{enumerate}[leftmargin=0.5cm, label=\arabic*.]
    \item Randomly sample a $b'$ from the $N_g$ registered users in the specified group. Generate a recursive PIR query for $b'$ and encrypt it using the originator's public key. Denote the encrypted query as $q'$.
    \item For each $i = 1, 2, \dots, n$ where $n$ is the number of lenders, generate a randomized ciphertext $c_i'$ that is of \type{1}.
    \item Generate a randomized commitment to $0$, denoted by $c_b'$, and sample a random number $\Delta r'$.
    \item According to $b'$ sampled above, choose the corresponding $s_{eb'}$ and calculate $y' = \text{PRF}_{s_{eb'}}(``y" \| r_e \| \text{date})$. Then use the public key of the originator to encrypt $y'$ and get a ciphertext $c'$. Generate a zero-knowledge proof $P_c'$ for the knowledge of the plaintext of $c'$.
    \item Generate the zero-knowledge proof $P_{form}'$ which proves that the query $q'$ is well-formed and the zero-knowledge proof $P_{corr}'$ which proves the correspondenceof $q'$ and $c'$.
    \item Generate a fake $t$ (denoted as $t'$) and a fake $X_b$ (denoted as $X_b'$). Simulate the process of the secure computation $f(X_b', t')$ to generate $\Lambda_{bf}'$ and $\Lambda_{of}'$.
    \item Output $(q', c_i'\text{'s}, \Delta r', c_b', c', P_c', P_{form}', P_{corr}', \Lambda_{bf}', \Lambda_{of}')$ to the exchanger.
\end{enumerate}
It is easy to see that the exchanger can get the same results (i.e. $``pass"$) from the zero-knowledge proofs of both simulation and real execution.
Also, we can see that every element in both $\text{View}_{ex}^{\pi}(\mathcal{I})$ and $\mathcal{S}_{ex}(r_e, s_{eu}\text{'s})$ is either a uniformly random number or a cryptographic primitive (such as a commitment, a ciphertext or zero-knowledge proof).
More importantly, every element is \emph{randomized independently} in both simultation and real execution. Therefore, under the assumption that the cryptographic primitives we use are correct and computationally indistinguishable (which also implies that known relations, e.g., the results of zero-knowledge proofs, stay the same), the two tuples which consist of independently randomized elements are also computationally indistinguishable, i.e., $\mathcal{S}_{ex}(r_e, s_{eu}\text{'s}) \approx \text{View}_{ex}^{\pi}(\mathcal{I})$.

\para{Originator. }
The originator is also involved in all the steps, and its view in the real execution is as follows: 
\begin{enumerate}[label={\alph*)}, leftmargin=0.5cm, itemsep=0pt, partopsep=0pt, parsep=0pt]
    \item During the secure aggregation: the mixture of the ciphertexts from the lenders and the noise from the exchanger (we denote the set of the mixtured responses as $C$), the commitment $c_b$ generated by the borrower, and $\Delta r = r_b - \sum r_i$ from the exchanger; \\
    \item During the anonymous authorization: the pseudo-random numbers $y_u$'s generated by the exchanger for the specified group; \\
    \item During the secure evaluation: the ciphertexts or commitments from the borrower to securely evaluate $f$, and we denote them as $\Lambda_{bf}$.\\
\end{enumerate}
We summarize the view of the originator as a tuple.
$\text{View}_{og}^{\pi}(\mathcal{I}) = (C, c_b, \Delta r, y_u\text{'s}, \Lambda_{bf})$.

And we construct a probabilistic-polynomial time simulator $\mathcal{S}_{og}$ that simulates the view of the originator using its input (namely $q, f$ and $t$) and output (namely $\textbf{n}$, $z_3$ and $z_4$). 
Similarly to $\mathcal{S}_{ex}$, we only consider the situation where the value of $z_3$ is $``pass"$, as a $\bot$ actually leads to a simpler case.
$\mathcal{S}_{og}$ works as follows:
\begin{enumerate}[leftmargin=0.5cm, label=\arabic*.]
    \item Generate a fake $X_b$ (denoted as $X_b'$) such that $f(X_b, t) = z_4$. Sample a random number $r_b'$ and generate a commitment $c_b'$ with randomness $r_b'$.
    \item According to $\textbf{n} = (n_0, n_1, \dots, n_d)$, generate $C_1', C_2', \dots, C_d'$ where $C_i'$ consists of $n_i$ ciphertexts of \type{i} using the public key of the originator.  Then sample $n_0$ commitment randomness $r_j' (j = 1, 2, \dots, n_0)$ and use them to generate $n_0$ commitments of $0$. Encrypt these commitments to $n_i$ ciphertexts of \type{0}.
    \item Sample $N_g$ random numbers, denoted as $y_u$'s.
    \item Simulate the secure computation process of $f$ using $X_b'$ and $t$ as inputs, and retrieve the message $\Lambda_{bf}'$ from the borrower.
    \item Output $(C', c_b', \Delta r', y_u'\text{'s}, \Lambda_{bf}')$ to the originator, where $C' = C_0' \cup C_1' \cup \dots \cup C_d'$ and $\Delta r' = r_b' - \sum r_j'$.
\end{enumerate}

Thus we have $\mathcal{S}_{og} = (C', c_b', \Delta r', y_u'\text{'s}, \Lambda_{bf}')$, and each item in $\mathcal{S}_{og}$ is independently randomized. 
Also, as long as the crytographic primitives of $\mathcal{S}_{og}$ is computationally indistinguishable, we can prove that $\mathcal{S}_{og}$ is computational indistinguishable with $\text{View}_{og}^{\pi}(\mathcal{I})$.

The views of the borrower and lenders are simple and the computational indistinguishability of their simulators and views are directly from existing cryptographic primitives such as PIR, GC and ZKP.

\para{Malicious participants. }
Malicious participants in our model may collude or send invalid messages. 
In \sysname, we use ZKPs and actively secure garbled circuits to prevent invalid messages. 
On the other hand, if the borrower and the originator collude, we can construct a simulator for the union of them and prove the security. The simulator can be constructed in a similar way as $\mathcal{S}_{og}$, as the borrower can only provide messages about her own input.
Actually, as the exchanger has checked the validity of the messages using ZKPs, the loan information of other borrowers are protected by Algorithm~\ref{algorithm:pir_sparse_recursive} and the noise generated by the exchanger. In fact, the only information the borrower can bring to the originator is her own loan information, which does not help the originator get other borrowers' loan information.
These simulators can be constructed similarly and we omit the details here.

\subsection{$\mathcal{F}_{loan}$ Meets Security Goals}
We proposed several security goals in Section~\ref{section:security_goal}.  We now show that $\mathcal{F}_{loan}$ achieves these goals. And as \sysname securely realizes $\mathcal{F}_{loan}$, \sysname achieves these security goals.

\emph{Anonymity} is achieved as $\mathcal{F}_{loan}$ does not reveal the borrower's identity to the exchanger or any lender.
Similarly, $\mathcal{F}_{loan}$ achieves \emph{Privacy-B} and \emph{Privacy-O} as $\mathcal{F}_{loan}$ does not reveal $x_{ib}$'s and $t$ to others.
Also, $\mathcal{F}_{loan}$ checks the validity of the query and the correspondence of the borrower's secret and the query while protecting the borrower's identity, thus it ensures \emph{Authorization}.

It remains to show that $\mathcal{F}_{loan}$ achieves \emph{Privacy-L}. Recall that $I_{ib'}$ is the indication that $x_{ib'} \ne 0$ for each borrower $b'$.
Actually, step 4 of $\mathcal{F}_{loan}$ makes the type of the response of a lender $S_i$ $(\epsilon, \delta)$-differentially private to the originator. The type of the response, however, reveals no more information than $I_{ib'}$, as $x_{ib'}$ is hidden by its commitment. Therefore, $I_{ib'}$ is at least $(\epsilon, \delta)$-differentially private to the originator.

